LLMs Can't Plan, But Can Help Planning in LLM-Modulo Frameworks

There is considerable confusion about the role of Large Language Models (LLMs) in planning and reasoning tasks. On one side are over-optimistic claims that LLMs can indeed do these tasks with just the right prompting or self-verification strategies. On the other side are perhaps over-pessimistic claims that all that LLMs are good for in planning/reasoning tasks are as mere translators of the problem specification from one syntactic format to another, and ship the problem off to external symbolic solvers. In this position paper, we take the view that both these extremes are misguided. We argue that auto-regressive LLMs cannot, by themselves, do planning or self-verification (which is after all a form of reasoning), and shed some light on the reasons for misunderstandings in the literature. We will also argue that LLMs should be viewed as universal approximate knowledge sources that have much more meaningful roles to play in planning/reasoning tasks beyond simple front-end/back-end format translators. We present a vision of {\bf LLM-Modulo Frameworks} that combine the strengths of LLMs with external model-based verifiers in a tighter bi-directional interaction regime. We will show how the models driving the external verifiers themselves can be acquired with the help of LLMs. We will also argue that rather than simply pipelining LLMs and symbolic components, this LLM-Modulo Framework provides a better neuro-symbolic approach that offers tighter integration between LLMs and symbolic components, and allows extending the scope of model-based planning/reasoning regimes towards more flexible knowledge, problem and preference specifications.

==> fine-tuning-and-synthetic-data-section.tex <==
\subsection{Fine Tuning \& Synthetic Data}
\label{sec:syntheticdata}

\donote{too long...}

Once the LLM-Modulo framework ``solves'' a planning instance, the solution can then be added to a synthetic data corpus (step 6 in Figure~\ref{fig:llm-modulo}), which is intermittently used to fine tune the LLM (step 7), so its future plan candidate guesses improve. 

Such fine tuning on task-specific data has been a  popular way to get LLMs to improve their performance on reasoning/planning tasks. For example, fine tune the LLM on blocks world planning problem-solution pairs to improve their performance in guessing solutions for blocks world instances
\cite{pallagani2023understanding}. While fine tuning still doesn't guarantee correctness of the generated solutions, it might improve the chances that LLM guesses candidates that are closer to being vetted by the bank of critics. 

One important question is where this additional data for fine tuning comes from. A tempting idea is to have the LLM itself generate this additional data, and improve it by self-critiquing/verification, before fine-tuning itself on the data. This EM-like approach unfortunately will not work given that LLMs can't verify their own solutions (see Section~\ref{sec:cantverify}). In the past, this meant that the only reliable way to generate synthetic data is to use external plan generators--for example, use a classical planner like FF \cite{hoffmann2001ff} to solve a host of blocks world instances and then use those solutions to fine-tune the LLM. 
%
The LLM-Modulo framework, in contrast, provides an alternative way of using an LLM-based framework to generate synthetic data that is guaranteed correct. 

%\rao{CRITICISM: This is perhaps unnecessary cirticism as fine turning anyway doesn't guarantee that LLMs will generate correct solutions.. so it is not like finetuning with not-fully-guaranteed-correct data is going change anything big.}

%\rao{Karthik/Kaya--write this self-improvement imfeasibility as a corollary of failure to verify}



==> travel-planner-table.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lc|cc|cc|c}
        \toprule
        \textbf{Model} & \multicolumn{1}{c}{\textbf{Delivery}} & \multicolumn{2}{c}{\textbf{Commonsense}} & \multicolumn{2}{c}{\textbf{Hard}} & \multicolumn{1}{c}{\textbf{Final Pass}} \\
         & \multicolumn{1}{c}{\textbf{Rate}} & \multicolumn{2}{c}{\textbf{Pass Rate}} & \multicolumn{2}{c}{\textbf{Pass Rate}} & \multicolumn{1}{c}{\textbf{Rate}} \\

        & \textbf{} & \textbf{Micro} & \textbf{Macro} & \textbf{Micro} & \textbf{Macro} & \textbf{} \\
        \midrule
        % Direct$_{\rm GPT-3.5-Turbo}$ & 0.99 & 0.61 & 0.03 & 0.11 & 0.03 & 0.00 \\
        Direct $_{\rm GPT-3.5-Turbo}$ & 99.4 & 61.5 & 3.9 & 11.2 & 2.8 & 0.0 \\
        % Direct$_{\rm GPT-4-Turbo}$ & 1.0 & 0.85 & 0.25 & 0.52 & 0.24 & 0.04 \\
        Direct $_{\rm GPT-4-Turbo}$ & 100 & 84.9 & 25.6 & 51.9 & 24.4 & 4.4 \\

        \textcolor{gray!75}{CoT$_{\rm GPT-3.5-Turbo}$} & \textcolor{gray!75}{\text{100}} & \textcolor{gray!75}{\text{66.3}} & \textcolor{gray!75}{\text{3.3}} & \textcolor{gray!75}{\text{11.9}} & \textcolor{gray!75}{\text{5}} & \textcolor{gray!75}0 \\
        \textcolor{gray!75}{ReAct$_{\rm GPT-3.5-Turbo}$} & \textcolor{gray!75}{\text{82.2}} & \textcolor{gray!75}{\text{47.6}} & \textcolor{gray!75}{\text{3.9}} & \textcolor{gray!75}{\text{11.4}} & \textcolor{gray!75}{\text{6.7}} & \textcolor{gray!75}{0.6} \\
        \textcolor{gray!75}{Reflexion$_{\rm GPT-3.5-Turbo}$} & \textcolor{gray!75}{\text{93.9}} & \textcolor{gray!75}{\text{53.8}} & \textcolor{gray!75}{\text{2.8}} & \textcolor{gray!75}{\text{11}} & \textcolor{gray!75}{\text{2.8}} & \textcolor{gray!75}{0} \\

        \textbf{LLM Modulo [All]$_{\rm GPT-3.5-Turbo}$} & \textbf{97.8} & \textbf{59.8} & \textbf{13.3} & \textbf{14} & \textbf{6.7} & \textbf{5} \\
        LLM Modulo [Common]$_{\rm GPT-3.5-Turbo}$ & 100 & 67.9 & 16.7 & 14 & 5 & 2.8 \\

        LLM Modulo [Hard]$_{\rm GPT-3.5-Turbo}$ & 100 & 61.3 & 4.4 & 10.7 & 5.6 & 1.6 \\
        LLM Modulo [Json]$_{\rm GPT-3.5-Turbo}$ & 100 & 61.3 & 4.4 & 10.2 & 3.9 & 1.1 \\
        \textbf{LLM Modulo [All]$_{\rm GPT-4-Turbo}$} & \textbf{100} & \textbf{89.2} & \textbf{40.6} & \textbf{62.1} & \textbf{39.4} & \textbf{20.6} \\
        \bottomrule
    \end{tabular}
    \caption{
    We report the results on TravelPlanning Validation set following \cite{xie2024travelplanner}. Grayed out results on CoT / ReAct / Reflexion variants are reported from \cite{xie2024travelplanner} for completeness. Direct$_{\text{Model}}$ are reproduced baselines as implemented in \cite{xie2024travelplanner}. $\text{LLM Modulo}[\text{Crtic}]_{\mathcal{M}}$ represents the critics used during the LLM-Modulo planning with model $\mathcal{M}$. Values are percentages of delivery rate, micro and macro commonsense and hard constraints and finally, success rate defined as \textit{Final Pass Rate} as in \cite{xie2024travelplanner}.
    }
    \label{fig:travel-planning}\label{tab:model_performance}
\end{table*}
